Unveiling and Consulting Core Experts in Retrieval-Augmented MoE-based LLMs

Retrieval-Augmented Generation (RAG) significantly improved the ability of Large Language Models (LLMs) to solve knowledge-intensive tasks. While existing research seeks to enhance RAG performance by retrieving higher-quality documents or designing RAG-specific LLMs, the internal mechanisms within LLMs that contribute to the effectiveness of RAG systems remain underexplored. In this paper, we aim to investigate these internal mechanisms within the popular Mixture-of-Expert (MoE)-based LLMs and demonstrate how to improve RAG by examining expert activations in these LLMs. Our controlled experiments reveal that several core groups of experts are primarily responsible for RAG-related behaviors. The activation of these core experts can signify the model's inclination towards external/internal knowledge and adjust its behavior. For instance, we identify core experts that can (1) indicate the sufficiency of the model's internal knowledge, (2) assess the quality of retrieved documents, and (3) enhance the model's ability to utilize context. Based on these findings, we propose several strategies to enhance RAG's efficiency and effectiveness through expert activation. Experimental results across various datasets and MoE-based LLMs show the effectiveness of our method.

==> tables/adjust_general.tex <==

\begin{table}[t!]
\centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule 
    \textbf{Method} & \textbf{Expert Type}& \textbf{PopQA} & \textbf{RGBqa} \\
    \midrule
   \textbf{No Adjustment} & None & 50.70 & 89.33 \\
    \midrule
   \multirow{2}{*}{\textbf{Enhancement}  $\uparrow$ } & Random & 50.03 & 88.00 & \\
   &General & \textbf{50.40} & \textbf{88.33} & \\
   % & General & x & x & \\
   \midrule
    \multirow{2}{*}{\textbf{Inhibition}  $\downarrow$ } & Random & 47.60 & 83.00 & \\
    & General & \textbf{13.40} & \textbf{38.33} \\
    % & General & x & x & \\
    \bottomrule
    \end{tabular}   }
    \caption{Results of adjusting expert activation on Mixtral-8x7B. Metric is exact match.}
        \vspace{-0.4cm}
    \label{tab:adjust_general}
\end{table}
